RGBD Objects in the Wild: Scaling Real-World 3D Object Learning from RGB-D Videos

We introduce a new RGB-D object dataset captured in the wild called WildRGB-D. Unlike most existing real-world object-centric datasets which only come with RGB capturing, the direct capture of the depth channel allows better 3D annotations and broader downstream applications. WildRGB-D comprises large-scale category-level RGB-D object videos, which are taken using an iPhone to go around the objects in 360 degrees. It contains around 8500 recorded objects and nearly 20000 RGB-D videos across 46 common object categories. These videos are taken with diverse cluttered backgrounds with three setups to cover as many real-world scenarios as possible: (i) a single object in one video; (ii) multiple objects in one video; and (iii) an object with a static hand in one video. The dataset is annotated with object masks, real-world scale camera poses, and reconstructed aggregated point clouds from RGBD videos. We benchmark four tasks with WildRGB-D including novel view synthesis, camera pose estimation, object 6d pose estimation, and object surface reconstruction. Our experiments show that the large-scale capture of RGB-D objects provides a large potential to advance 3D object learning. Our project page is https://wildrgbd.github.io/.

==> tables/depth_est.tex <==

\begin{table}[t]
%     \setlength\tabcolsep{0.05em} % default value: 6pt
    \label{tab:depth_est}
    \vspace{-2mm}
    \resizebox{0.48\textwidth}{!}{
    \centering
    \begin{tabular}{l|c|l|c}
    \toprule
        Method (novel views) &  MAE$\downarrow$/SD & Method (known views) & MAE$\downarrow$/SD \\
        \midrule
         NeRF~\cite{mildenhall2020nerf}  & 0.306/0.109   & NeuS~\cite{wang2021neus} &  \textbf{0.535}/0.152  \\
         Mip-NeRF 360~\cite{barron2022mip}  & \textbf{0.185}/0.068    & VolSDF~\cite{yariv2021volume} & 0.643/0.048  \\
         Instant-NGP~\cite{muller2022instant}  & 0.366/0.105  & Neusfacto~\cite{Yu2022SDFStudio} & 0.717/0.171  \\
    \bottomrule
    \caption{\textbf{RGB depth estimation results.} {Average of depth MAE are reported with their standard deviation (SD). We train NeRF-series methods  only in training split but SDF-series methods in all splits.}}
    \end{tabular}
    }

\end{table}
